The Internet of Things in the Era of Generative AI: Vision and Challenges

Advancements in Generative AI hold immense promise to push Internet of Things (IoT) to the next level. In this article, we share our vision on IoT in the era of Generative AI. We discuss some of the most important applications of Generative AI in IoT-related domains. We also identify some of the most critical challenges and discuss current gaps as well as promising opportunities on enabling Generative AI for IoT. We hope this article can inspire new research on IoT in the era of Generative AI.

==> Section/2_background.tex <==
\section{BACKGROUND OF GENERATIVE AI}
\label{sec:background}
\vspace{-0mm}
%% P1:
% - Definition of Generative AI
% - Examples of traditional generative models
% - Examples of contemporary generative models
%
Generative AI refers to AI models that can generate new content in the form of text, images, videos, codes, and many more. Generative models are not new. Although traditional generative models such as Recurrent Neural Networks (RNN),  Variational Autoencoders (VAE), Generative Adversarial Networks (GAN), and Bidirectional Encoder Representations from Transformers (BERT) have found their applications in a variety of domains, it is until recently that billion-parameter generative models such as GPT series, DALL-E series, and LLaMA series marked a significant breakthrough. These models demonstrated remarkable performance across a wide spectrum of tasks, elevating the capabilities of Generative AI to unprecedented levels.
%series have made the breakthrough and achieved remarkable performance in a wide range of tasks.
 
%such as chat and search, image synthesis, software programming, and music composition~\cite{agi_application_2023}. 
%, compared to their predecessors, such as BERT~\cite{bert_2019} or GAN.

%% P2: Talk about the key characteristics of contemporary generative models. 

The superiority of the contemporary generative models can be attributed to the following two key characteristics:

\begin{itemize}
\item\textbf{Significantly Large Model Size:} 
Contemporary generative models contain significantly more parameters than the traditional ones. For example, GPT-4 contains about 1.8 trillion parameters, which is 5,000 times larger than BERT. 
%This exponential increase not only greatly enhances the existing capabilities of contemporary generative models~\cite{scaling_model_2022}, but also give them some emergent abilities that were unattainable with previous small models~\cite{emergent_2022}.

\vspace{1mm}
\item\textbf{Pre-trained on Massive Amount of Data:} Contemporary generative models are pre-trained on much larger datasets than their predecessors. For example, GPT-4 is pre-trained on more than 500 billion tokens that are over one hundred times than BERT. 
\end{itemize}
\vspace{1mm}
%% P3: Talk about the key capabilities of contemporary generative models brought by the characteristics. These capabilities serve as the basis for Section 3 and 4.
These characteristics equip contemporary generative models with some unique abilities that were not attainable before:

\begin{itemize}
\item\textbf{Generating High-Quality Data:} Compared to traditional generative models, the quality of content generated by contemporary generative models is significantly improved. For example, DALL-E 2 is able to generate images that are high in detail and produce visually compelling results that can be indistinguishable from photographs taken by cameras or created by artists.
%witnessed exponential growth, enabling the synthesis of realistic and coherent data. 

%These models leverage the attention mechanism of transformer models in conjunction with recent innovations like latent diffusion to generate new content with far better realism in a flexible end-to-end manner. This is in contrast to previous generation models based on Generative Adversarial Networks (GANs) which relied on a more rigid training structure specifically designed for a particular use-case. The use of transformers makes these models particularly versatile as they can be adopted for a wide range of tasks and are particularly suited for multi-modal applications due to the use of cross-attention, unlike traditional models like GANs.  The use of positional embeddings and the attention mechanism allow these models to generate more detailed and high-resolution content. 
\vspace{1mm}
\item{
\textbf{Tackling Complex Tasks with Human-Level Performance:} Contemporary generative models are capable of tackling more complex tasks that conventional counterparts are difficult to deal with. For instance, given a task description along with a brief prompt that contains a few training samples, contemporary generative models such as GPT-4 demonstrate the capability of solving complicated mathematical problems with accuracy comparable to human performance.
}
%which is far beyond the reach of earlier, smaller language models such as Bert~\cite{bert_2019}.
% Emergent abilities refer to the abilities that are not present in smaller models but are present in larger models~\cite{emergent_2022}. 
%Modern large-scale generative have been observed to perform well under the few-shot prompting setting, where the pre-trained model is given a \textit{prompt} containing a natural language instruction of a task with a few input-output examples in the model’s context as a preamble, and completes the response to the unseen examples. Additionally, these contemporary models are also capable of further improving their performance under this setting with some external strategies, such as leveraging explanations in the prompting, utilizing instructions during fine-tuning, and guiding them to produce a sequence of intermediate steps before giving the final answer(chain-of-thought). Both of these two capabilities are generally regarded as the unique \textit{emergent ability}~\cite{emergent_2022} of the modern large-scale generative models.
\vspace{1mm}
\item{
\textbf{Superior Generalization Capability:} 
% Contemporary generative models accumulates much more knowledge than the old ones due to the fact that they have learned from massive amount of data during the pre-training phase~\cite{scaling_data_2022}. This gives them the ability to tackle a wider range of real-world situations even in a zero-shot way. As a result, their generalization capability is better than the older generative models that require frequent fine-tuning to fit new tasks or out-of-distribution data.
Contemporary generative models exhibit superior generalization ability on new tasks and data. For example, conventional generative models such as GAN require retraining or fine-tuning to generate images that belong to different domains. In contrast, DALL-E 2 is able to generate images for domains that have not been trained before.
}
%without the need for frequent parameter adjustment.
% accumulates much more knowledge than the old ones due to the fact that they have learned from massive amount of data during the pre-training phase~\cite{scaling_data_2022}. This gives them the ability to tackle a wider range of real-world situations even in a zero-shot way. As a result, their generalization capability is better than the older generative models that require frequent fine-tuning to fit new tasks or out-of-distribution data.

% As demonstrated by prior research~\cite{scaling_data_2022}, large-scale models can continuously accumulate knowledge and improve their final behavior when exposed to extensive training data. Consequently, contemporary generative models that are trained on datasets comprising even trillions of data points often acquire the robustness to address a broader spectrum of real-world scenarios even in a zero-shot way, thus establishing their superior generalization capabilities compared with their predecessors. For instance, compared to the traditional image generation models, such as GAN~\cite{gan_2014}, which require frequent fine-tuning to fit different scenarios, recent DALL-E 2~\cite{dall-e-2_2022} is able to generate images that are even not present in its large-scale pre-trained dataset, based on the user's preference.
\end{itemize}


%In the following sections, we use Generative AI to refer to contemporary generative models.


% \vspace{-1mm}
% With these two unique abilities, modern generative models can produce personalized content such as texts, speech, video, and images in higher quality according to user-defined instructions or prompts, which is difficult to accomplish with old small-scale models. Consequently, these large-scale generative models yield more satisfying results and even enable the execution of many complex tasks through these emergent abilities. For instance, given a brief prompt that contains a few training samples and a task description, recent generative language models such as GPT-4~\cite{gpt4_2023} demonstrate an impressive ability to solve mathematical problems and generate programming code with accuracy comparable to human performance, which is far beyond the reach of earlier, smaller language models such as Bert~\cite{bert_2019}.

%%
% Contemporary generative models possess some emergent abilities that were achievable with previous models. This is due to their exponential increase in model parameters, which not only enhances their existing capabilities~\cite{scaling_model_2022}, but also provides them with some new ones~\cite{emergent_2022}. For example, modern generative models can produce personalized content such as texts, speech, video, and images in high quality according to user-defined instructions or prompts, which is difficult to accomplish with old small-scale models. Consequently, these large-scale generative models yield more satisfying results and even enable the execution of many complex tasks through these emergent abilities. For instance, given a brief prompt that contains a few training samples and a task description, recent generative language models such as GPT-4~\cite{gpt4_2023} demonstrate an impressive ability to solve mathematical problems and generate programming code with accuracy comparable to human performance, which is far beyond the reach of earlier, smaller language models such as Bert~\cite{bert_2019}.

% Contemporary generative models, especially those leveraging latent diffusion principles, have reshaped our understanding of AI's potential. These models introduce noise to input data meticulously, transforming it into white noise. The subsequent reversal of this process enables the accurate recreation of the original data. This intricate methodology presents a solution to the persistent issue of mode collapse commonly found in GANs~\cite{gan_2014}. While many GAN-derived results tend to have a blurry appearance, diffusion models consistently produce sharp and detailed outputs. Coupling these models \cite{yang2022diffusion} with powerhouses like BERT~\cite{bert_2019} or GPT-3~\cite{gpt-3_2020}, that rely on the newly developed attention-based transformer architecture~\cite{vaswani2017attention} and have been trained on vast amounts of data, has resulted in generating exceptionally high-quality text. Newer iterations, such as GPT-4~\cite{gpt4_2023}, with even larger model sizes, have surpassed previous benchmarks, showcasing unparalleled abilities in tasks like problem-solving, code-generation, and multi-domain content creation, outpacing earlier models like BERT~\cite{bert_2019}. 

% Furthermore, the scope of content that contemporary generative models can produce is staggering. While GANs primarily focus on generating visual content like images, modern generative models extend their dominion to texts, codes, music, and more. This vastness in content range allows for broader applicability in industries ranging from entertainment to IoT.




% The generalization capability of current generative models is also better than the old ones. This superiority comes from the fact that they are pre-trained on substantially larger datasets than their predecessors. As demonstrated by prior research, large-scale models can continuously assimilate knowledge and improve their final behavior when exposed to extensive training data~\cite{scaling_data_2022}. Consequently, contemporary generative models that are trained on datasets comprising trillions of data points often acquire the robustness to address a broader spectrum of real-world scenarios even without necessitating fine-tuning, thus establishing their superior generalization capabilities compared with their predecessors. For instance, compared to the traditional image generation models, such as GAN~\cite{gan_2014}, which require frequent fine-tuning to fit different scenarios, recent DALL-E 2~\cite{dall-e-2_2022} is able to generate images that are even not present in its large-scale pre-trained dataset, based on the user's preference.

% \noindent\textbf{Better Generalization Capability:} 
% Modern large language models stand as monolithic architectures, embodying the culmination of rigorous training on colossal textual datasets. This extensive training enables them to capture and reproduce the intricate patterns characteristic of human language. In contrast to GANs~\cite{gan_2014}, which often falter in maintaining coherence over longer text sequences, these titan models effortlessly craft intricate narratives, crossing varied domains, styles, and tones, and even show evidence of logical reasoning about new problems~\cite{liu2023evaluating}. Their adaptability further shines when integrated with external knowledge bases, marrying creativity with informational accuracy. Such models also embrace an interactive generation mode, welcoming real-time feedback, and enabling a more harmonious human-AI collaboration. This intensive training regime, coupled with the ability to absorb and generalize across vast datasets, sets them leagues apart from their predecessors. For instance, while traditional models like GANs~\cite{gan_2014} often necessitated fine-tuning to adapt to varying scenarios, next-gen models like DALL-E 2~\cite{dall-e-2_2022} exhibit an uncanny ability to generate images beyond their training scope, precisely tailored to user preferences.

% What sets these newer generative AI models apart is their versatility and ability to perform a wide array of creative tasks. They can generate coherent text, create high-quality images from textual descriptions, perform image classification, and much more, all while exhibiting a deeper understanding of context and semantics. The introduction of self-attention mechanisms and transformer architectures has played a pivotal role in achieving these advancements.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Draft
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Generative AI in the realm of the Internet of Things (IoT) is designed to produce data or content pertinent to IoT devices, networks, and their applications. It is emblematic of a burgeoning domain that merges the creativity of generative AI with the pervasive nature of IoT. For applications like predictive maintenance, anomaly detection, and network optimization, older models such as Generative Adversarial Networks (GANs) have historically been employed. However, the landscape has shifted with the advent of newer generative AI techniques tailored for IoT environments.

% Recent innovations like ChatGPT~\cite{gpt-3_2020} and DALL-E 2~\cite{dall-e-2_2022} have established the foundation for the latest wave of generative AI for IoT. The distinction between these new approaches and previous models, including GANs, lies in two primary aspects:

% \textbf{(1) Exponential Increase in Model Parameters:} Newer generative models for IoT applications have adopted an architectural scale much grander than their predecessors. It has been observed that the sheer augmentation in the number of model parameters can lead to unexpected yet beneficial emergent properties~\cite{emergent_2022}. By scaling from millions to several billions of parameters, these models can not only interpret vast IoT data streams effectively but also exhibit adaptive behaviors, ranging from real-time optimization to intricate task solutions for IoT ecosystems.

% \textbf{(2) Enhanced Data Handling and Superior Generalization:} The training datasets for modern generative models have grown exponentially, especially in the context of IoT where data streams are ceaseless and varied. It's corroborated by studies that even more modestly sized models exhibit remarkable performance enhancements when trained with vast datasets, in alignment with certain scaling laws~\cite{scaling_data_2022}. In the contemporary IoT context, these models, armed with knowledge from trillions of data points, can adeptly navigate diverse real-world scenarios. Their broad learning base, coupled with the specialized nature of IoT data, ensures unparalleled generalization abilities, often surpassing the constraints of older generation models like GANs.

